AxisGuide: Grounding Robot Action Coordinate System in RGB Observations for Robust Visuomotor Manipulation

Visuomotor manipulation policies trained via large-scale behavior cloning have achieved strong semantic scene understanding, yet often fail to reliably execute correct low-level actions under distribution shifts. For example, even in a simple pickup task with identical scene layouts, camera viewpoints, and illumination, performance can degrade substantially when the object is placed at unseen locations. We argue that this gap arises from insufficient action understanding, namely the inability to interpret the robot's base-frame action coordinate system in image space. To address this issue, we introduce AxisGuide, a lightweight guidance method that bridges semantic scene understanding and action-coordinate interpretation. Using camera parameters and end-effector poses, AxisGuide renders the robot base-frame axes in each camera view and augments RGB observations with a small set of cue channels that explicitly visualize the meaning of the +x, +y, and +z motions in image space. Extensive evaluations in both the LIBERO simulation and real-world environments demonstrate that AxisGuide yields substantial performance gains and improved generalization, highlighting the effectiveness of explicit action-coordinate cues for learning reliable and transferable generalist visuomotor policies.

==> figs/rollout2.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=1.0\textwidth]{figs-pdf/rollout_tmp2.pdf}
  \caption{rollout example}
  \label{fig:multi-view libero performance}
\end{figure*}

==> sec/8_rebuttal.tex <==
This author response corresponds to Paper-ID [\textbf{526}]. We sincerely thank the area chair and reviewers for their thoughtful and constructive feedback. We will revise the presentation details (e.g., figures) noted by the reviewers.
\vspace{0.1em}
% \jy{TODO: we provide reviewers feedback~ or authors ~ }
% We denote previous references by placing a bar over citation numbers (e.g., [$\bar{1}$])
% We thank the reviewers for their valuable feedback. They noted that our approach provides insight into the ``action understanding gap'' (\revA{W7KQ}, \revB{JDES}), is simple and efficient (\revA{W7KQ}, \revB{JDES}), and generalizes well to unseen spatial arrangements (\revC) with strong interpretability (\revA{W7KQ}). We address their concerns below.
% We thank the reviewers for their constructive feedback and address the main concerns below.
% As the reviewers pointed out, our method requires camera calibration, and some degree of error is inevitable in real-world deployment. We would first like to emphasize that even in our real-world experiments, the calibration process is not noise-free: the estimated extrinsic matrices already contain small inaccuracies. Nevertheless, our method consistently improves performance across many experiments and demonstrates strong robustness in practice.


% We would first like to emphasize that the real-world results reported in our paper were already obtained under imperfect calibration. In practice, the estimated camera parameters contained small inaccuracies, e.g., the slight gripper misalignment visible in the supplementary video. 

\noindent[\ac{}, \revA{}, \revC, \revB{}] \textbf{System calibration sensitivity.} We highlight that our real-world experiments in manuscript already contain unavoidable system calibration noise, and our method still consistently improves performance across experiments. We further evaluate the robustness of our method to projection errors caused by inaccurate system calibrations on the \textbf{Novel Object Position (NOP)} task in Fig.~5 (manuscript). In the table below, we report results under extrinsic (left) and intrinsic (right) perturbations at inference time, while using a model trained with unperturbed camera parameters. Errors in robot kinematics and EEF pose estimations are reflected in this experiment, since they also perturb the projected EEF position.
These results demonstrate our method's \textbf{robustness to realistic calibration noise}, as performance degrades marginally and still exceeds the baseline [23] performance of 52.4 reported under unperturbed settings. We will include this experiment in the revised manuscript.
\begin{table}[h]
  \centering
  \vspace{-0.3cm}
  \setlength{\tabcolsep}{3.5pt}
  \renewcommand{\arraystretch}{0.8}
  \scriptsize
  \label{tab:calib_sensitivity}
  \begin{tabular}{ccccc|cccc}
    \toprule
     \diagbox[height=1.6em]{\raisebox{-0.6ex}{\scriptsize Rot.}} {{\scriptsize Trans.}}  & 0 cm & 1 cm & 2 cm & 3 cm & \diagbox[height=1.5em]{\raisebox{-0.6ex}{\scriptsize Focal.}}{\scriptsize P.P.} & 0 px & 5 px & 10 px \\
    \midrule
    0$^\circ$ & \textbf{65.7} & 64.3 & 61.9 & 62.4 
    & 0\% & \textbf{65.7} & 63.8 & 65.2 \\
    3$^\circ$ & 64.8 & 64.8 & 62.9 & 61.4 
    & 5\% & 64.3 & 63.8 & 65.2 \\
    6$^\circ$ & 64.3 & 64.8 & 64.3 & 63.3 
    & 10\% & 64.3 & 64.3 & 63.8 \\
    \bottomrule
  \end{tabular}
  % {\raggedright\scriptsize \tiny $^{*}$ All results in this sensitivity analysis use the 90k-step checkpoint for consistency, yielding a clean extrinsic baseline of 67.1. The main paper instead reports 65.7, which is based on the 100k-step checkpoint used for the final results.\par}
  \vspace{-0.39cm}
\end{table}

\noindent[\ac{}, \revB{}] \textbf{Additional baselines.} To compare our method with other visual cues, we evaluate TraceVLA~[$30$] and AimBot~[$4$] as suggested by the reviewer, on \textbf{NOP} task.
% We compare our method with prior image-cue baselines.
% TraceVLA and AimBot aim to improve scene understanding by providing visual cues that encode the spatial relationship between the object and the end-effector. However, successful task execution in novel environments requires more than understanding the spatial relationship. The policy must also determine what action to take in the novel scene, which requires understanding the robot’s action coordinate system in image space. While TraceVLA and AimBot enrich the observation with scene-level spatial cues, they are not specifically designed to explicitly represent the robot’s action coordinate system. As a result, when the object appears in unseen locations, these methods offer limited guidance on how the policy should adjust its actions, making improvements under distribution shift difficult. 
% In contrast, by explicitly grounding the robot’s action coordinates in the visual observation and showing where the $x$, $y$, and $z$ action directions lie in the image, 
% AxisGuide helps the policy infer how to move toward a target even under novel object positions. This leads to larger gains in \textbf{table above} and enables more reliable, robust manipulation. We will include this comparison in the revised manuscript.
These methods improve scene understanding by providing visual cues about the spatial relationship between the object and the EEF. However, successful execution in novel situations requires not only scene understanding but also an understanding of the robot’s base-frame in image space. Since these baselines are not specifically designed to represent the robot's action coordinate system, they provide limited guidance for actions when objects appear in unseen locations.
In contrast, AxisGuide explicitly grounds the robot’s action coordinates in the image. This helps the policy infer how to move toward the target under novel object positions, leading to larger gains in the table below and more reliable, robust manipulation. We will include this comparison in the revised manuscript.
\begin{table}[h]
  \centering
  \setlength{\tabcolsep}{7pt}
  \renewcommand{\arraystretch}{0.2}
  % \captionsetup{font=scriptsize}
  % \caption{Generalization to novel object position with additional baselines.}
  \scriptsize
  \vspace{-0.3cm}
  \label{tab:r2}
  \begin{tabular}{cccc}
    \toprule
    SmolVLA [23] & [23] + TraceVLA [30]  & [23] + AimBot [4]& [23] + Ours \\
    \midrule
    52.38 & 51.90 & 52.38 & \textbf{65.71} \\
    \bottomrule
  \end{tabular}
  \vspace{-0.4cm}
\end{table} 
% As shown in Table \ref{tab:r2}, our method demonstrates greater robustness under unseen object locations compared to AimBot and TraceVLA. 



% Although these methods facilitate scene understanding by providing visual cues about the spatial relationship between objects and the end-effector (Sec.~\Romannum{2}.B), they do not provide any guidance on how this understanding can be translated into concrete actions.
% %The image-level cues alone may be insufficient for precise action adjustments under spatial variations. 
% In contrast, our method interprets this relationship from an action-oriented perspective. By explicitly grounding the robot's action coordinate system in the visual observation, our approach produces more reliable action adjustments, leading to robust behavior even under distribution shifts.

% \jy{
% \noindent\textbf{Additional baselines.}
% We compare our method with prior image-cue baselines on the [Task Name] task (Table R2).
% As shown in Table~R2, both AimBot and TraceVLA often fail to reach the object under unseen object locations, whereas our method remains more robust. We believe this result highlights that, for robust manipulation, it is not sufficient to provide only image-level spatial cues; explicitly conveying action-relevant information is also critical.

% As discussed in Sec.~II.B, both TraceVLA and AimBot also attempt to provide spatial cues about the relationship between the object and the end-effector. However, these methods primarily target spatial relationships as they appear in image space. In contrast, our method interprets this relationship from the perspective of action, by explicitly grounding the robot's action coordinate system in the observation.

% }


% We believe this performance gap arises because the magnitude of the projected vector varies significantly depending on the relative position of the end-effector with respect to the camera, i.e., how far the end-effector is from the camera. In contrast, normalized vectors provide a more consistent representation of direction regardless of the end-effector position. We believe this makes policy learning more stable, as the model can rely on a direction cue that is less affected by changes in camera-relative distance. For this reason, we use unit vectors as the default setting.
% At the same time, we agree that vector magnitude may also carry meaningful information, as it could reflect how large the actual movement is in the image. We believe that designing a better way to preserve and utilize such magnitude information is an interesting direction for future work.

% \noindent[\revA{}] \textbf{Applicability to dynamic environments.} As the reviewer pointed out, mobile-base and eye-in-hand settings can introduce additional challenges because the projected action axes continuously change due to base motion and viewpoint variation. Nevertheless, as also shown in the supplementary video for the wrist-camera setting, the results in Table~II and Fig.~3 of the manuscript demonstrate that our method maintains stable performance despite these continuous changes. We believe this suggests that in such settings, where continuous base motion makes the action–image relationship harder to interpret, explicitly indicating the underlying action coordinate system, that is, what motion along the +x, +y, and +z axes means in the image becomes even more important. \yj{In these setting, continuous base motion makes the action--image relationship harder to interpret. We believe this result suggests that in such settings, explicitly indicating the underlying action coordinate system, that is, what motion along the +x, +y, and +z axes means in the image becomes even more important.}  While alternative frames (e.g., end-effector or object-centric frames) may provide more stable cues, as the reviewer mentioned, they are misaligned with the policy's action frame, making it more difficult to relate the action space to image observations.

% \noindent[\revA] \textbf{Conflicting guidance.}
% We would like to emphasize that our guidance is not intended to provide a trajectory for task success, but rather to represent an explicit association between the action space and the image observation, that is, how motion along the +x, +y, and +z axes appears in the image. In addition, the guide may not create conflicting signals with RGB observations since we never trained the model to output actions that follow the drawn arrows. We believe that strong performances on LIBERO-Goal and LIBERO-Long as shown in Fig.~3 of the manuscript as an experimental response to the reviewer’s concern, where the policy must detour obstacles to accomplish some tasks (e.g., moving a plate to the front of the stove).
\vspace{0.1em}
\noindent[\revC] \textbf{Aliasing error.}
% \jy{To analyze aliasing, we consider the standard setting where both the robot base frame and the camera pose are fixed. Under this assumption, the projection from the base-frame coordinate system to the image is uniquely determined under the pinhole camera model [7]. In particular, distinct canonical action directions in the base frame are mapped to distinct directions in image space, so aliasing does not arise at this stage. Assuming a pinhole camera, we then examine whether aliasing error can occur in each of the following three stages.}
Assuming a pinhole camera, we project 3D coordinates into the 2D image through three stages. We examine whether aliasing can occur at each stage for projections of the robot’s base-frame action directions from arbitrary EEF positions. (1) The first stage projects 3D points onto the image planes at each point’s depth $Z$, using the camera parameters. These points are the EEF point and three additional points obtained by applying unit canonical actions as noted in Sec \Romannum{3}-C. By definition [7], this projection is a one-to-one mapping, so aliasing error cannot occur. (2) The second stage maps the projected points onto the image plane at unit depth by applying $1/Z$ to each point according to its depth.
Because all the canonical unit moves in our method have consistent magnitudes, which is not proportional to depth, this stage does not introduce aliasing. 
We then use these points to define 2D direction vectors corresponding to the +x, +y, and +z action directions. 
(3) The final stage rescales the 2D direction vectors to unit length. 
% Aliasing errors can arise here when vectors that were previously distinguished by depth normalization become indistinguishable after rescaling. However, because such situations are rare in practice, aliasing in our method is not critical to performance and can even be beneficial, as demonstrated by the ablation results in the table below.
Aliasing errors can arise here when vectors previously distinguished by depth normalization become identical after rescaling, but such situations are rare in practice. This is supported by the table below, where using normalization leads to better performance. \begin{wraptable}[3]{l}{0.5\linewidth} 
\vspace{-0.4cm}
    \centering
    \setlength{\tabcolsep}{3pt}
    \renewcommand{\arraystretch}{0.6}
    % \captionsetup{font=scriptsize}
    % \caption{Ablation on vector normalization.}
    \scriptsize
    \label{tab:r3}
    \begin{tabular}[t]{lcc} 
      \toprule
      LIBERO Task & Ours & Unnormalized \\
      \midrule
      Pick \& Place (Bowl) & \textbf{88.0} & 85.3 \\
      Stove (Long)  & \textbf{78.7} & 74.7 \\
      \bottomrule
    \end{tabular}
    \vspace{-0.3cm}
\end{wraptable}
% In addition, the results in Tables \Romannum{1} and \Romannum{2} (main paper) show that our baseline KYC~[$12$] that doesn't have aliasing error at the representational level, do not necessarily achieve superior performance. Our method outperforms KYC, which represents 3D camera geometry using Plücker rays and employs an additional model to encode them.
% \jy{In addition, our method outperforms KYC~[$12$] in Tables \Romannum{1} and \Romannum{2}, even though KYC avoids aliasing error at the representational level by encoding 3D camera geometry with Plücker rays using an additional model.}
Moreover, using representations without aliasing error (e.g., quaternions) doesn't necessarily achieve superior performance. Tables \Romannum{1} and \Romannum{2} (manuscript) show that our method outperforms KYC~[$12$], which uses additional encoder for 3D camera geometry.
  
\vspace{0.1em}
\noindent[\revB] \textbf{Ablation on projected vector normalization.} As shown in the table above, normalizing the projected vectors to unit length yields better performance. We believe that reducing the variance in the length of projected vector helps stabilize policy learning by allowing the model to focus on direction, because the length of the projected vectors varies significantly with the depth of the EEF.
\vspace{0.1em}

\noindent[\revB{}] \textbf{Model parameter and latency.} 
As shown in supplementary materials, the increase in the number of model parameters and the additional inference time are minimal.
% \ws{Summarize contents in supplementary materials and then refer reviewer to there}

% We provide the detailed efficiency analysis in the supplementary material. In brief, in the multi-view SmolVLA setting, AxisGuide adds only \textbf{0.590M} parameters over the \textbf{450.046M} parameters of the vanilla model (\textbf{+0.13\%}) and incurs only \textbf{+5.41 ms} additional latency per inference (batch=1), including cue generation and channel-wise concatenation.

%\noindent[\revB{}] \textbf{Presentation details.} We will revise the figure and typo to address this concern. 
% In line with the reviewer’s comment, altering the y-axis of the figure may introduce bias. 

\vspace{0.1em}
\noindent[\revA{}] \textbf{Applicability to dynamic environments.} 
% As the reviewer pointed out, mobile-base and eye-in-hand settings are particularly challenging because continuous base motion and viewpoint changes constantly modify the action–image relationship, making it more difficult for the policy to infer this relationship from images alone.
Mobile-based and eye-in-hand settings can be more challenging for visuomotor policies, as continuous base motion and viewpoint changes constantly alter the action-image relationship. 
We believe this is where explicitly grounding the action coordinate system on the observation can be helpful. As shown in the supplementary wrist-camera video, Table~II, and Fig.~3 (manuscript), our method maintains stable performance despite these continuous changes in the projected action axes and outperforms  baselines. 
% This suggests that, when the action–image relationship becomes harder to interpret, explicitly showing where the +x, +y, and +z action directions lie in the image may provide useful guidance to the policy.
% More broadly, robust mobile manipulation under base motion is an important future direction. Furthermore, as the reviewer noted, alternative frames such as end-effector-centric or object-centric coordinates may provide more stable cues. Exploring how to combine such stability with explicit grounding of the policy’s action space would be a promising avenue for future work.
We believe that extending our method to mobile manipulation and to alternative frames such as EEF-/object-centric coordinates would be valuable future work.


\vspace{0.1em}
\noindent[\revA{}] \textbf{Conflicting guidance.} We emphasize that the guide is unlikely to conflict with RGB observations, which is supported by the robust performance on LIBERO-Goal/-Long in Fig.~3 (manuscript), where the success often requires detouring around obstacles. This is because our guide represents how motion along the +x, +y, and +z axes appears in the image, rather than indicating a direct path for task success. 
% Moreover, we don't train the model to produce actions that follow these arrows.

%In addition, the reviewer suggested an idea of training an encoder that uses a representation inherently immune to aliasing error. KYC, which is our baseline in Table \Romannum{1} and \Romannum{2}, adopts such approach. KYC represents 3D camera geometry using Plücker rays and employs an additional model to encode them. However, as stated in our manuscript, our method outperforms KYC in all experiments. In summary, aliasing error is not highly critical in practice, and methods that eliminate aliasing error at the representational level do not necessarily achieve better performance.


%We explicitly inform the policy how the robot base frame appear in the 2D observation. To implement this, we assume a pinhole camera [$\bar{7}$], under which the 3D-to-2D projection consists of projecting 3D coordinates onto the image plane using the camera parameters, followed by depth normalization with respect to their depths. We project the three canonical unit moves defined along the robot base-frame axes and rescale each projected vector to unit length. For any two camera setups, the projected canonical unit moves cannot share the same directions, because the projection defined by the camera parameters is, by definition, a one-to-one mapping [$\bar{7}$]. In addition, for any two distinct 3D points under a fixed viewpoint, the projected moves originating from these points cannot become identical in the image plane because all the three canonical unit moves have the same fixed magnitude in 3D. Thus, any aliasing in our method can only arise from the subsequent rescaling of these projected vectors to unit length. However, according to the ablation results in~\cref{tab:r3}, its impact on performance is not significant. \jy{TODO: add to mention comparison with KYC.}

% Therefore, aliasing error can only occur in the specific case where two parallel vectors originate from two 3D points on the same ray passing through the pinhole, are projected to have the same length due to depth normalization.

%In perspective projection, points that lie on the same ray are mapped in a many-to-one manner. However, since the policy is designed to output actions based on 2D inputs, what matters to us is not the 3D action coordinate vector direction itself, but rather how it appears in 2D. Therefore, if we explicitly distinguish between 3D vectors that overlap when projected into 2D, this may introduce additional information that we did not intend, potentially leading to an inconsistent representation. This is why we adopted the current approach.

%Moreover, reviewer VHrh proposed a potential remedy for this information loss by suggesting an encoder training methodology which directly feeds 3D information into the model. However, the KYC baseline used in our paper already adopts a similar approach, which trains an additional encoder to embed camera parameters represented using Plücker rays. Based on the KYC results in Table \Romannum{1} and \Romannum{2} where our method outperforms the KYC baseline, it appears that fully preserving all 3D information may be detrimental.

% \jy{
% \noindent \textbf{Information loss.}
% We would like to clarify that perspective projection itself does not inherently introduce aliasing for the geometric relationship that our cue is designed to encode. Under a calibrated pinhole camera, the cue is constructed by projecting a fixed reference point together with the endpoints of the three action-axis directions. In this sense, the cue preserves how the robot action coordinate system appears in the image, rather than attempting to represent arbitrary 3D scene geometry. Perspective projection maps 3D points to the image through camera intrinsics and extrinsics, and camera pose is recovered in standard pose-estimation formulations from known 3D--2D correspondences. ~\cite{cameraSpaceAction} (we need to change)

% The ambiguity arises only after we normalize the projected axis vectors. Normalization intentionally removes magnitude information and keeps only direction. Under perspective projection, points lying on the same camera ray share the same image direction structure, since points of the form $\lambda P$ project to the same image location in normalized coordinates. Therefore, after normalization, aliasing can occur for points that differ primarily by translation along the same camera ray.~\cite{cameraSpaceAction} (we need to change)

% However, this is a highly restricted degeneracy rather than broad information collapse. The ambiguous set is generically confined to a one-dimensional ray through the camera center, not a broad subset of the 3D workspace. In other words, normalization discards radial scale, but it still preserves the angular information that determines how the action axes appear in the image, which is the quantity our method is designed to convey. Empirically, this design is also beneficial: as shown in Table~R3, the normalized version performs better than the unnormalized one, suggesting that removing unstable magnitude variation improves robustness in practice.
% }

%To this end, we project the three canonical unit moves defined along the robot base-frame axes from the current EEF gripper center, into the 2D observation and then normalize them to unit vectors. 
\vspace{0.1em}
\noindent[\revA{}] \textbf{Scope.} As the reviewer insightfully noted, aspects such as force control or tactile feedback, which are not directly related to the action coordinate system, are outside our scope. 
% While our approach may be described as ``reaching'',
We view accurate understanding of the action coordinate system as a fundamental component, as many manipulation failures stem from \textbf{misaligned action interpretation} rather than downstream fine-grained interaction. Our key point is that improving action-coordinate understanding leads to consistent gains across diverse tasks and settings, suggesting that it plays a broadly important role in visuomotor manipulation.
% We do not regard axisguide as a silver bullet for generalizability.\jy{is it ok to use the word 'silver bullet' ?} Instead, we believe that improving the generalizability of reaching substantially contributes to the overall generalizability of a manipulation policy, because all the elements such as force control, tactile feedback, and object properties become meaningless if reaching itself is not performed correctly. \jy{meaningless is not proper. it's aggressive} As suggested, we will carefully review the manuscript and adjust any parts that may overstate the contribution of Axisguide.
% We do not view AxisGuide as a complete solution to all aspects of generalization in manipulation. \yj{Do we need this sentence?} Instead, 
% AxisGuide is designed to help policies better understand the robot's action coordinate system from image observations, which in turn improves reaching and spatial action grounding. We believe this is an important component of robust manipulation, since successful manipulation usually requires first reaching the correct location with the correct motion direction.
% Among the various components that constitute manipulation, aspects such as force control, tactile feedback, and object properties that are not related to the action coordinate system are outside the scope of the problems we aim to address. Moreover, our approach has demonstrated its effectiveness not only in simple reaching but also on all the LIBERO suites that require diverse actions. This shows that understanding the action coordinate system is crucial for improving the generalizability of the broad range of manipulation subtasks.

%AxisGuide is designed to help policies better understand the robot’s action coordinate system from image observations, thereby improving spatial action grounding. We agree that AxisGuide is not intended to explicitly model all aspects of manipulation, such as force control or tactile feedback. Understanding action coordinate system is a fundamental component of manipulation, since many manipulation tasks require the policy to correctly interpret how to move in 3D space before grasping, placing, or interacting with objects. Consistent with this, our experiments are not limited to isolated reaching, but demonstrate improvements across diverse LIBERO manipulation tasks, including long-horizon settings. We therefore view AxisGuide as a broadly applicable module for improving action understanding in visuomotor manipulation.

%so that only the level of importance we genuinely intend to claim is emphasized.



==> tabels/location_generalizability_results.tex <==
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.2}
\begin{table}[t]
  \centering
  \caption{Quantitative results on generalizability on new object location in pick up task}
  \label{tab:new_object_location}
  \begin{tabular}{llc}
    \toprule
    Environment & Method & Pick up object \\
    \midrule
    \multirow{2}{*}{Real-world} 
      & DP~\cite{diffusionpolicy}              & 30.12 \\
      & DP + AxisGuide (Ours)\textbf{ }                             & \textbf{50.00} (\red{19.88$\uparrow$}) \\
    \midrule
    \multirow{2}{*}{Simulation}  
      & Smolvla~\cite{smolvla}              & 37.14 \\
      & Smolvla + AxisGuide (Ours)                             & \textbf{58.57} (\red{21.43$\uparrow$}) \\
    \bottomrule
  \end{tabular}
\end{table}

==> tabels/multi_view_simul_results.tex <==
\begin{table}[t]
  \centering
  \caption{Quantitative results on multi-view (wrist-mounted cam and front cam)  visuomotor policy performance in LIBERO~\cite{libero} simulation \jy{convert this table as figure(graph) with DP, Smolvla}}
  \label{tab:multi_view_main}
  \begin{tabular}{lcccc}
    \toprule
    Method & spatial task 0 & goal task 0 & object 4 & 10 task 2\\
    \midrule
    DP~\cite{diffusionpolicy} & 74.67 & 90.67 & 100.0 & 74.67 \\
    DP + Ours & 88.00 (\red{13.33$\uparrow$}) & 90.67 (\red{0.00$\uparrow$})& 100.0 (\red{00.00$\uparrow$})& 78.67 (\red{4.00$\uparrow$})\\
    \bottomrule
  \end{tabular}
\end{table}
